Efficient Non-Learning Similar Subtrajectory Search

Similar subtrajectory search is a finer-grained operator that can better capture the similarities between one query trajectory and a portion of a data trajectory than the traditional similar trajectory search, which requires the two checked trajectories are similar to each other in whole. Many real applications (e.g., trajectory clustering and trajectory join) utilize similar subtrajectory search as a basic operator. It is considered that the time complexity is O(mn^2) for exact algorithms to solve the similar subtrajectory search problem under most trajectory distance functions in the existing studies, where m is the length of the query trajectory and n is the length of the data trajectory. In this paper, to the best of our knowledge, we are the first to propose an exact algorithm to solve the similar subtrajectory search problem in O(mn) time for most of widely used trajectory distance functions (e.g., WED, DTW, ERP, EDR and Frechet distance). Through extensive experiments on three real datasets, we demonstrate the efficiency and effectiveness of our proposed algorithms.

==> expectedMCF.tex <==
\section{Minimum Cost Assignment with Expected Distances}

==> proposedSolution1.tex <==
\section{Exact Similar Subtrajectory Search Algorithms}
In this section, we briefly introduce the basic exact algorithm for the SSS problem and the framework of our algorithm in this paper.
\subsection{Basic Solution}
The vast majority of distance functions~\cite{YiJF98, ChenN04, ChenOO05, KoideXI20, VlachosGK02, 0007BCXLQ18, Yuan019, Xie14, AltG95} are defined via dynamic programming processes. ExactS~\cite{WangLCL20} is proposed to solve the similar sub-trajectory search problem in $O(mn)$ time complexity based on this point. For two trajectories $\tau_q$ and $\tau_d[i:\tau_d.l]$, we can compute a similarity matrix $M$ by dynamic programming $DP$, where $M_{x,y}$ denotes the distance between $\tau_q[1:x]$ and $\tau_d[i:i+x-1]$. In this process, $\Theta(\tau_q,\tau_d[i:i+x])$ can be computed from $\Theta(\tau_q, \tau_d[i:i+x-1])$ in $O(1)$ time~\cite{WangLCL20}.


\begin{algorithm}[t]
	{\small
	\DontPrintSemicolon
	\KwIn{\small a query trajectory $\tau_q$, a data trajectory $\tau_d$}
	\KwOut{\small a sub-trajectory $\tau_d[i^{*},j^{*}]$}
    $i^{*}\gets 0, j^{*}\gets 0$\;
    $score\gets \infty$\;
    \ForAll{$1\leq i \leq \tau_d.l$}{
        $M\gets DP(\tau_q,\tau_d[i:\tau_d.l])$\;
        $y^{*} \gets \mathop{\arg\min}\limits_{ 1\leq y\leq \tau_d.l-i+1}{M_{\tau_q.l,y}}$\;
        \If{$M_{\tau_q.l,y^{*}}<score$}{
            $score\gets M_{\tau_q.l,y^{*}}$\;
            $i^{*}\gets i$\;
            $j^{*}\gets y^{*} + i - 1$\;
        }
    }
    \Return{$\tau_d[i^{*},j^{*}]$}
	\caption{\small $ExactS(\tau_q,\tau_d)$}
	\label{algo:efficiencyE}}
\end{algorithm}
The time complexity of solving the distance between trajectories by dynamic programming is {\small$O(\tau_q.l\cdot\tau_d.l)$}. Therefore, ExactS can be applied to most of the distance functions. However, $DP$-based ExactS is difficult to achieve {\small$O(\tau_q.l\cdot\tau_d.l)$} in terms of time complexity.

\subsection{Matching Algorithm}
This section will discuss how to find the subtrajectory with the shortest distance to the query trajectory from the data trajectory for a given query trajectory $\tau_q$ and a data trajectory $\tau_d$. Although previous work \cite{WangLCJ19} has optimized the time complexity of this problem to {\small$O(\tau_q.l\cdot\tau_d.l^2)$}, it still makes the computational cost increase dramatically when the length of the data trajectory is large. This paper reduces this time complexity to {\small$O(\tau_q.l\cdot\tau_d.l)$} by a dynamic programming algorithm.



Distinguishing from existing algorithms, the algorithm proposed in this paper is not based on the existing dynamic programming method for calculating the distance. Instead, the basic idea of the algorithm is to calculate the minimum cost of converting the points in the query trajectory to the data trajectory by three operations: insertion, deletion, and substitution. Each point in the query trajectory is converted to its matching point in the data trajectory at a specific cost in the conversion process. 

In Example \ref{exa:wed_example}, we transform the trajectory $\tau_q$ into $\tau_d$ by several operations. There are two possible transformations for each point in $\tau_q$: deletion or substitution. For each substituted point in $\tau_q$, we can easily find a point in $\tau_d$ to match it. On a different note, for each deleted point, it is difficult to find a match; for example, there is no match for a point $\tau_q[2]$ in Example \ref{exa:wed_example}. Therefore, we assume that each deleted point matches the same point as its predecessor, e.g., point $\tau_q[2]$ matches point $\tau_d[1]$ as well as point $\tau_q[1]$. Then, we give the formal definition of matching.
\begin{definition}[Match]
	Given two trajectories $\tau_q$ and $\tau_d$, in the process of transforming $\tau_q$ into $\tau_d$, $\tau_q[i]$ and $\tau_d[j]$ are matched if and only if one of the following two cases is satisfied.
	\begin{enumerate}
		\item $\tau_q[i]$ is substituted with $\tau_d[j]$ and $\tau_d[j]$ has not been substituted.
		\item $\tau_q[i]$ is deleted and $\tau_q[i-1]$ is a match to $\tau_d[j]$.
	\end{enumerate}
\end{definition}

\noindent\textbf{Conversion Cost.} After defining the concept of matching, we can analyze the \textit{conversion cost} for each point in the query trajectory to its matching point in the data trajectory.
When $\tau_q[i]$ matches $\tau_d[j]$, depending on the different matches of $\tau_q[i-1]$, we define three different conversion costs $Cost_{sub}$, $Cost_{ins}$ and $Cost_{del}$ and give the demenstration of these conversion costs in Figure \ref{fig:conversion_cost}:\\
(1) $\tau_q[i-1]$ matches $\tau_d[j]$. This means that we need to remove $\tau_q[i]$, and we denote the conversion cost as $Cost_{del}(\tau_q[i], \tau_d[j])$. \\(2) $\tau_q[i-1]$ matches $\tau_d[j-1]$. In this case, $\tau_q[i]$ will be replaced with $\tau_d[j]$, and we will denote this conversion cost as $Cost_{sub}(\tau_q[i], \tau_d[j])$. \\ 
(3) $\tau_q[i-1]$ matches $\tau_d[k]$, where $1\neq k<j-1$. For this situation, we should not only substitute $\tau_q[i]$ with $\tau_d[j]$, but also insert $\tau_d[k+1:j-1]$. We denote the conversion cost as $Cost_{ins(k)}(\tau_q[i], \tau_d[j])$.



\begin{figure}[t!]
	\centering
	\subfigure[][{\scriptsize $Cost_{del}$}]{
		\scalebox{0.06}[0.06]{\includegraphics{../figures/del.png}}
		\label{fig:del}}
	\subfigure[][{\scriptsize $Cost_{sub}$}]{
		\scalebox{0.06}[0.06]{\includegraphics{../figures/sub.png}}
		\label{fig:sub}}
	\subfigure[][{\scriptsize $Cost_{ins}$}]{
		\scalebox{0.06}[0.06]{\includegraphics{../figures/ins.png}}
		\label{fig:ins}}
	\caption{\small Demonstration of the conversion cost}
	\label{fig:conversion_cost}
\end{figure}
% For example, finding the subtrajectory from $\tau_d$ with the smallest distance to $\tau_q$ is equivalent to the smallest cost of the summation of conversion cost for each point in $\tau_q$ to its matching point in $\tau_d$.

\noindent\textbf{Calculate $C_{i,j}$.} We denote by $C_{i,j}$ the minimum value of the cost of converting $\tau_q[1:i]$ into $\tau_d[1:j]$ when $\tau_q[i]$ matches $\tau_d[j]$. We will discuss the computation process of $C_{i,j}$ in three cases. \\
\textbf{(1) $i=1$.}
When $i=1$, we should substitute $\tau_q[1]$ with $\tau_d[j]$. Therefore, $C_{i,j}=Cost_{sub}(\tau_q[i], \tau_d[j])$.\\
\textbf{(2) $j=1$.}
There are two possible ways of converting $\tau_q[i]$ when $j=1$: deleting $\tau_q[i]$, which means that $\tau_q[i-1]$ matches $\tau_d[1]$ so that we have $C_{i,j}=C_{i-1,j}+Cost_{del}(\tau_q[i], \tau_d[j])$; the other way is to substitute $\tau_q[i]$ with $\tau_d[1]$, which means that $\tau_q[1:i-1]$ will be deleted, resulting in $C_{i,j}=Cost_{sub}(\tau_q[i], \tau_d[j])+\sum_{k=1}^{i-1}Cost_{del}(\tau_q[k], \tau_d[j])$. Therefore, we have $C_{i,j}=\min \{C_{i-1,j}+Cost_{del}(\tau_q[i], \tau_d[j]), Cost_{sub}(\tau_q[i], \tau_d[j])+\sum_{k=1}^{i-1}Cost_{del}(\tau_q[k], \tau_d[j])\}$.\\
\textbf{(3) $1<i\neq \tau_q.l,1<j\neq \tau_d.l$.}
Considering that the point $\tau_q[i]$ matches $\tau_d[j]$, there are three different conversion possibilities for $\tau_q[i]$ and $C_{i,j}=\min\{delCost,subCost,insCost\}$:
\begin{enumerate}
    \item $delCost_{i,j}$: deleting $\tau_q[i]$. When $\tau_q[i]$ is deleted, by the definition of matching, $\tau_q[i-1]$ and $\tau_d[j]$ are matched and we have $delCost_{i,j}=C_{i-1,j}+Cost_{del}(\tau_q[i], \tau_d[j])$.
    \item $subCost_{i,j}$: substituting $\tau_q[i]$ with $\tau_d[j]$. In this case, $\tau_q[i-1]$ matches $\tau_d[j-1]$ and we have $subCost_{i,j}=C_{i-1,j-1}+Cost_{sub}(\tau_q[i], \tau_d[j])$.
    \item $insCost_{i,j}$: substituting $\tau_q[i]$ and inserting $\tau_d[k+1:j-1]$. In this situation, $\tau_q[i-1]$ may match $\tau_d[k]$ ($1\leq k<j-1$). We should insert $\tau_d[k+1:j-1]$ and have $C_{i,j}=C_{i-1,k}+Cost_{ins(k)}(\tau_q[i], \tau_d[j])$. Considering all possible values of $k$, $insCost_{i,j}=\min_{1\leq k<j-1} C_{i-1,k}+Cost_{ins(k)}(\tau_q[i], \tau_d[j])$.
\end{enumerate}
\noindent In case 3.2, our substitution of $\tau_q[i]$ for $\tau_d[j]$ can be seen as inserting an empty string along with the substitution. Therefore, we will discuss 3.2 and 3.3 together in the subsequent sections.

Once we have calculated $C_{i,j}$, the distance between the query trajectory and the optimal sub-trajectory is the minimum conversion cost when $\tau_q[\tau_q.l]$ matches a point in the data trajectory, i.e., $\mathop{\min}\limits_{1\leq i \leq j \leq \tau_d.l}{\Theta( \tau_q,\tau_d[i:j])}=\mathop{\min}\limits_{1\leq j \leq \tau_d.l}C_{\tau_q.l,j}$.

To obtain the starting position $i^{*}$ and ending position $j^{*}$ of the optimal subtrajectory, we use $S_{i,j}$ to mark the position of the point that matches $\tau_q[1]$ in $\tau_d$ when $\tau_q[i]$ matches $\tau_d[j]$. Based on the computation process of $C_{i,j}$, we are able to determine which point $\tau_q[i-1]$ matches when $\tau_q[i]$ matches $\tau_d[j]$. Suppose $\tau_q[i-1]$ matches $\tau_d[k]$ ($1\leq k\leq j$), then we have $S_{i,j}=S_{i-1,k}$. Finally, the Matching Algorithm (MA) \ref{algo:efficiencyA} is proposed to solve the SSS problem.

\noindent\textbf{Complexity.} Since $Cost_{sub}(\tau_q[i], \tau_d[j])$ and $Cost_{del}(\tau_q[i], \tau_d[j])$ involve only the substitution and deletion of one trajectory point, their time complexity is $O(1)$; therefore, when $i=1$, the time complexity of $C_{i,j}$ is $O(1)$. We can calculate $\sum_{k=1}^{i-1}Cost_{del}(\tau_q[k], \tau_d[j])$ when $j=1$ in advance for any $i$ by preprocessing, and thus we can compute $C_{i,j}$ within the time complexity of $O(1)$. In other cases, we need to calculate $\min\{delCost,subCost,insCost\}$. Given the specific distance function, we will discuss in Section \ref{sec:solution1} how to compute $C_{i,j}$ in $O(1)$ time complexity. Therefore, the time complexity of MA is {\small$O(\tau_q.l\cdot\tau_d.l)$}.


\begin{algorithm}[t]
	{\scriptsize
	\DontPrintSemicolon
	\KwIn{\small a query trajectory $\tau_q$, a data trajectory $\tau_d$}
	\KwOut{\small a sub-trajectory $\tau_d[i^{*},j^{*}]$}
    \ForAll{$1\leq i \leq \tau_q.l$}{
        \ForAll{$1\leq j \leq \tau_d.l$}{
            \uIf{$i=1$}{
                $C_{i,j}\gets Cost_{sub}(\tau_q[i], \tau_d[j])$\;
                $S_{i,j}\gets j$\;
            }\ElseIf{$j=1$}{
                $C_{i,j}=\min \{C_{i-1,j}+Cost_{del}(\tau_q[i], \tau_d[j]),$ $ Cost_{sub}(\tau_q[i], \tau_d[j])+\sum_{k=1}^{i-1}Cost_{del}(\tau_q[k], \tau_d[j])\}$\;
                $S_{i,j}\gets 1$\;
            }\Else{
                $C_{i,j}=\min\{delCost_{i,j},subCost_{i,j},insCost_{i,j}\}$\;
                update $S_{i,j}$ according to the matches of $\tau_q[i-1]$\;
            }
        }
    }
    $j^{*}\gets \mathop{\arg\min}\limits_{j}C_{\tau_q.l,j}$\;
    $i^{*}\gets S_{\tau_q.l,j^{*}}$\;
    \Return{$\tau_d[i^{*},j^{*}]$}
	\caption{\small $MA(\tau_q,\tau_d)$}
	\label{algo:efficiencyA}}
\end{algorithm}


\section{Details of the Algorithm Design}
\label{sec:solution1}

In this section, we will discuss how to calculate the conversion cost and $C_{i,j}$ for each point of the query trajectory when using the two different distance functions, WED and DTW.
\subsection{Minimum Cost of WED}
By introducing the concept of matching, we can convert the distance between trajectories into the cost required to convert points in $\tau_q$ into points in $\tau_d$. Let's discuss the cost of converting each point $\tau_q[i]$ to the point $\tau_d[j]$ it matches in $\tau_d$. \\
\textbf{Conversion Cost.} 
(1) $\tau_q[i-1]$ matches $\tau_d[j]$. We should delete $\tau_q[i-1]$ so that $Cost_{del}(\tau_q[i], \tau_d[j])=del(\tau_q[i])$. \\
(2) $\tau_q[i-1]$ matches $\tau_d[j-1]$. We should substitute $\tau_q[i]$ with $\tau_d[j]$, i.e., $Cost_{sub}(\tau_q[i], \tau_d[j])=sub(\tau_q[i],\tau_d[j])$. \\
(3) $\tau_q[i-1]$ matches $\tau_d[k]$, where $1\neq k<j-1$. The cost of converting $\tau_q[i]$ to $\tau_d[j]$ is the summation of $sub(\tau_q[i], \tau_d[j])$ and the cost of inserting the trajectory $\tau_d[k+1:j-1]$. Therefore, we have $Cost_{ins(k)}=ins(\tau_d[k+1:j-1])+sub(\tau_q[i],\tau_d[j])$.


\begin{example}
	Consider the example in Figure \ref{fig:wed_example}, where $\tau_q$ is converted into $\tau_d$. Since $\tau_q[1]$ has no predecessor node, $\tau_q[1]$ is only substituted for $\tau_d[1]$ with the cost of $sub(\tau_q[1],\tau_d[1])$. $\tau_q[2]$ matches $\tau_d[1]$, but since $\tau_q[1]$ matches $\tau_d[1]$, $\tau_q[2]$ has to be deleted, with the cost of $del(\tau_q[2])$. $\tau_q[4]$ matches $\tau_d[4]$ and $\tau_q[3]$ matches $\tau_d[2]$, thus $\tau_q[4]$ is converted to $\tau_d[4]$ with the cost of $sub(\tau_q[4],\tau_d[4])+ins(\tau_d[3])$.
\end{example}

\noindent \textbf{Calculate $C_{i,j}$.} After obtaining the conversion cost of the points using WED as a distance function, we can calculate $C_{i,j}$. We will discuss the relational equation for $C_{i,j}$ in three cases.\\
\textbf{(1) $i=1$.} $C_{i,j}=sub(\tau_q[1],\tau_d[j])$.\\
\textbf{(2) $j=1$.} $C_{i,j}=\min\{C_{i-1,j}+del(\tau_q[i]), sub(\tau_q[i],\tau_d[1])+del(\tau_q[1:i-1])\}$. \\
\textbf{(3) $1<i<\tau_q.l,1<j<\tau_d.l$.}
Considering that the point $\tau_q[i]$ matches $\tau_d[j]$, $\tau_q[i]$ may need to be deleted or substituted. Thus, the update of $C_{i,j}$ depends mainly on whether $\tau_q[i]$ is deleted or replaced.
\begin{enumerate}
    \item $delCost$. When $\tau_q[i]$ is deleted, by the definition of matching, $\tau_q[i-1]$ and $\tau_d[j]$ are matched and we have $delCost=C_{i-1,j}+del(\tau_q[i])$.
    \item $subCost$ and $insCost$. $\tau_q[i-1]$ may match $\tau_d[k]$ ($1\leq k<j-1$) while substituting $\tau_q[i]$. In this case, we should insert $\tau_d[k+1:j-1]$ and have $C_{i,j}=C_{i-1,k}+ins(\tau_d[k+1:j-1])+sub(\tau_q[i],\tau_d[j])$. Considering all possible values of $k$, $insCost=\min_{1\leq k<j-1} C_{i-1,k}+ins(\tau_d[k+1:j-1])+sub(\tau_q[i],\tau_d[j])$. Another situation is that $\tau_q[i-1]$ matches $\tau_d[j-1]$ and we have $subCost=C_{i-1,j-1}+sub\left(\tau_q[i],\tau_d[j]\right)$. Combining these two situation, we have $C_{i,j}=\min\{insCost,$ $subCost\}=\min_{1\leq k <j} C_{i-1,k}+ins(\tau_d[k+1:j-1])+sub(\tau_q[i],\tau_d[j])$. Then, the calculation of $C_{i,j}$ can be simplified by follows:
{\small\begin{align*}
    C_{i,j}&=\min_{1\leq k<j} C_{i-1,k}+ins\left(\tau_d[k+1:j-1]\right)\\
	       &+sub\left(\tau_q[i],\tau_d[j]\right) \label{equ:e1}\\
    &=\min \{\min_{1\leq k<j-1}C_{i-1,k}+ins\left(\tau_d[k+1:j-1]\right) \\
	&+sub\left(\tau_q[i],\tau_d[j]\right),C_{i-1,j-1}+sub\left(\tau_q[i],\tau_d[j]\right)\}\\
    &=\min\{C_{i,j-1}+ins\left(\tau_d[j-1]\right)-sub\left(\tau_{q}[i],\tau_d[j-1]\right)\\
    &+sub\left(\tau_{q}[i],\tau_d[j]\right),C_{i-1,j-1}+sub\left(\tau_q[i],\tau_d[j]\right)\}
\end{align*}}

\end{enumerate}

By the above analysis, we can obtain the expression for the calculation of $C_{i,j}$ while using WED as distance function
{\small\begin{equation}
C_{i,j}=\left\{
\begin{array}{ll}
sub(\tau_q[i],\tau_d[j]), & i=1 \\
\min\{C_{i-1,j}+del(\tau_q[i]), sub(\tau_q[i],\tau_d[1])\\
+del(\tau_q[1:i-1])\}, & j=1,i\neq1 \\
\min\{C_{i-1,j}+del(\tau_q[i]),\\
C_{i,j-1}+ins\left(\tau_d[j-1]\right)-\\
sub\left(\tau_{q}[i],\tau_d[j-1]\right)+sub\left(\tau_{q}[i],\tau_d[j]\right),\\
C_{i-1,j-1}+sub\left(\tau_q[i],\tau_d[j]\right)\},& otherwise
\end{array}
\right.
\label{eq:wed_cal}
\end{equation}}
\begin{figure*}[t!]
	\centering
	\subfigure[][{\scriptsize $C_{i,j}$}]{
	    \scalebox{0.12}[0.12]{
		    \includegraphics{../figures/demenstration.png}
	        \label{fig:cost_matrix}
	    }\vspace{1ex}
	}
	\subfigure[][{\scriptsize $S_{i,j}$}]{
		\scalebox{0.12}[0.12]{
			\includegraphics{../figures/demenstration2.png}
		    \label{fig:start_matrix}
		}
	}
	\caption{\small Demonstration of Calculating $C_{i,j}$ and $S_{i,j}$}
	\label{fig:demonstration}\vspace{-2ex}
\end{figure*}

Finally, we describe how the algorithm works using an example as follows.
\begin{example}
	Given two strings $\tau_q=aab\dots$ and $\tau_d=bac\dots$, we need to find the subtrajectory from $\tau_d$ that is closest to $\tau_q$. The insertion, deletion, and substitution costs are the same as the settings for example \ref{exa:wed_example}. At the beginning, we will initialize $C_{1,j}$ (i.e., $C_{1,j}=sub(\tau_q[1],\tau_d[j])$). Then initialize $C_{i,1}$ based on whether $\tau_q[i]$ matches $\tau_d[1]$. Figure \ref{fig:cost_matrix} shows that $\tau_d[1]=b$, thus only $\tau_q[3]$ is substituted with it. For $\tau_q[4]$, when it matches $\tau_d[8]$, we need to determine which point is optimal for $\tau_q[3]$ to match with. From Figure \ref{fig:cost_matrix}, we can see that the cost of $\tau_q[3]$ when matching with $\tau_d[6]$ is 0, being the minimum, which means we need to insert $\tau_d[7]$. Therefore, considering $\tau_q[4]=\tau_d[8]$, we can compute the result of {\small$C_{4,8}$ from $C_{3,6}$, i.e., $C_{4,8}=C_{3,6}+ins(\tau_d[7])+sub(\tau_q[4],\tau_d[8])=0+1+0=1$}. In the actual implementation of the algorithm \ref{algo:efficiencyA}, we will compute $C_{4,8}$ by $C_{4,7}$, i.e. {\small$C_{4,8}=C_{4,7}+ins(\tau_d[7])-sub(\tau_q[4],\tau_d[7])+sub(\tau_q[4 ],\tau_d[8])=1+1-1+0=1$}.

	On the other hand, the algorithm updates $S_{i,j}$ as it executes. For example, when $\tau_q[4]$ matches $\tau_d[8]$, $\tau_q[3]$ is matched with $\tau_d[6]$ and we have $S_{4,8}=S_{3,6}$ as shown in Figure \ref{fig:start_matrix}.
\end{example}


\subsection{Minimum Cost of DTW}
Unlike WED, the cost required to delete a point or insert a point in DTW is different, which can make the computation of $C_{i,j}$ a little difficult. Firstly, we should analyze the cost of converting each point $\tau_q[i]$ in the query trajectory to the point $\tau_d[j]$ it matches in the data trajectory.\\
\textbf{Conversion Cost.} (1) $\tau_q[i-1]$ matches $\tau_d[j]$. When $\tau_q[i]$ matches $\tau_d[j]$, the cost of deleting $\tau_q[i]$ is equal to the cost of substituting $\tau_q[i]$ with $\tau_d[j]$, thus we have {\small$Cost_{del}(\tau_q[i], \tau_d[j])=sub(\tau_q[i],\tau_d[j])$}. \\
(2) $\tau_q[i-1]$ matches $\tau_d[j-1]$. We should substitute $\tau_q[i]$ with $\tau_d[j]$, i.e., $Cost_{sub}(\tau_q[i], \tau_d[j])=sub(\tau_q[i],\tau_d[j])$. \\
(3) $\tau_q[i-1]$ matches $\tau_d[k]$, where $1\neq k<j-1$. The cost of converting $\tau_q[i]$ to $\tau_d[j]$ is the summation of $sub(\tau_q[i], \tau_d[j])$ and the cost of inserting the trajectory $\tau_d[k+1:j-1]$. The cost for inserting subtrajectories $\tau_d[k+1:j-1]$ depends on the points matched by $\tau_d[k]$ and $\tau_d[j]$ at $\tau_q$. Suppose $\tau_q[i-1]$ matches $\tau_d[k]$, then $\tau_q[i]$ will be matched into $\tau_d[j]$. Thus, the cost to insert $\tau_d[k+1:j-1]$ is {\small$\mathop{\min}\limits_{k\leq t\leq j-1}\sum_{p=k+1}^{t}{sub(\tau_q[i-1],\tau_d[p])}+\sum_{p=t+1}^{j-1}{sub(\tau_q[i],\tau_d[p])}$}. Therefore, we have $Cost_{ins(k)}=\mathop{\min}\limits_{k\leq t\leq j-1}\sum_{p=k+1}^{t}{sub(\tau_q[i-1],\tau_d[p])}+$ $\sum_{p=t+1}^{j-1}{sub(\tau_q[i],\tau_d[p])}+sub(\tau_q[i],\tau_d[j])$.

\begin{example}
    Let's take \ref{fig:example2} as an example, the cost of converting $\tau_q[1]$ to $\tau_d[1]$ when $i=1$ and $j=1$ is {\small$sub(\tau_q[1],\tau_d[1])=sub(b,b)$}. When $i=2$ and $j=1$, $\tau_q[2]$ can only be converted to $\tau_d[1]$, thus the cost of the conversion is {\small$sub(\tau_q[2],\tau_d[1])=sub(b,b)$}. By the time $\tau_q[4]$ matches $\tau_q[2]$, we need to delete $\tau_q[4]$ requiring a cost of {\small$del(\tau_q[4])=sub(\tau_q[4],\tau_q[2])$} because $\tau_q[3]$ matches $\tau_q[2]$. For i=9 and j=9, since $\tau_q[8]$ matches $\tau_d[7]$, the cost of converting $\tau_q[9]$ to $\tau_d[9]$ consists of not only the cost of the substitution $sub(\tau_q[9],\tau_d[9])$, but also the cost of inserting $\tau_d[8]$, that is, $\mathop{\min}\limits_{7\leq t\leq 8}\sum_{p=8}^{t}{sub(\tau_q[8],\tau_d[p])}$ $+\sum_{p=t+1}^{8}{sub(\tau_q[9],\tau_d[p])}$. It is equal to $\min\{sub(\tau_q[8],\tau_d[8]),sub(\tau_q[9],\tau_d[8])\}$. It can be understood in another way that when $\tau_q[8]$ matches $\tau_d[7]$ and $\tau_q[9]$ matches $\tau_d[9]$, inserting $\tau_d[8]$ is equivalent to replacing $\tau_d[8]$ with $\tau_q[8]$ or $\tau_q[9]$.
\end{example}


\textbf{Calculate $C_{i,j}$.} After analyzing the conversion cost, similarly, we discuss the computation of $C_{i,j}$ in three cases.\\
\textbf{(1) $i=1$.}
When $i=1$, $\tau_q[1]$ can only be substituted with $\tau_d[j]$ as the same as WED and we have {\small$C_{i,j}=sub(\tau_q[1],\tau[j])$}.\\
\textbf{(2) $j=1$.}
Considering that the cost of deleting $\tau_q[i]$ and substituting $\tau_q[i]$ is the same when $j=1$, we have
{\small
\begin{eqnarray}
    C_{i,j}&=&\min \{Cost_{sub}(\tau_q[i], \tau_d[j])+\sum_{k=1}^{i-1}Cost_{del}(\tau_q[k], \tau_d[j]), \notag\\
    &&C_{i-1,j}+Cost_{del}(\tau_q[i], \tau_d[j])\} \notag\\
    &=&\min \{\sum_{k=1}^{i}sub(\tau_q[k], \tau_d[j]), C_{i-1,j}+sub(\tau_q[i],\tau_d[1])\}\notag\\
    &=&C_{i-1,j}+sub(\tau_q[i],\tau_d[1]) \notag
\end{eqnarray}}
\noindent\textbf{(3) $1<i<\tau_q.l,1<j<\tau_d.l$.}
If we delete $\tau_q[i]$, we have $delCost=C_{i-1,j}+sub(\tau_q[i], \tau_q[j])$. Another conversion is substitution. $\tau_q[i-1]$ may be matched with any $\tau_d[k]$ ($1\leq k<j$), and $C_{i,j}$ denotes the smallest of all possible values. Thus, we have
{\small
\begin{eqnarray}
C_{i,j}&=& \min\{insCost, delCost\}\notag\\
&=&\min \{\min_{1\leq k<j-1} C_{i-1,k}+Cost_{ins(k)}(\tau_q[i], \tau_d[j]),\notag \\ 
&&C_{i-1,j-1}+Cost_{sub}(\tau_q[i],\tau_d[j])\}\notag \\
&=&\mathop{\min}\limits_{1\leq k<j}C_{i-1,k}+\mathop{\min}\limits_{k\leq t< j-1 }\sum_{p=k+1}^{t}{sub(\tau_q[i-1],\tau_d[p] )}\notag \\
&+&\sum_{p=t+1}^{j-1}{sub(\tau_q[i],\tau_d[p])}+sub(\tau_q[i],\tau_d[j])\notag \\
&=&\mathop{\min}\limits_{1\leq k<j}\mathop{\min}\limits_{k\leq t< j-1 }C_{i-1,k}+\sum_{p=k+1}^{t}{sub(\tau_q[i-1],\tau_d[p] )}\notag \\
&+&\sum_{p=t+1}^{j-1}{sub(\tau_q[i],\tau_d[p])}+sub(\tau_q[i],\tau_d[j]) \notag
\end{eqnarray}}
The time complexity of computing $C_{i,j}$ ($1<i<\tau_q.l, 1<j<\tau_d.l$) directly from the above expression is very high, and therefore we are required to simplify the computation of $C_{i,j}$ by theorem \ref{the:simplify}.
\begin{theorem}
\label{the:simplify}
    When $i\geq 2,j\geq 2$, we have $C_{i,j}=\mathop{\min}\limits_{1\leq k < j}C_{i-1,k}+\sum_{t=k+1}^{j}sub(\tau_q[i], \tau_d[t])$.
\end{theorem}
\begin{proof}
    We will use mathematical induction to prove this theorem. To simplify the proof, we temporarily denote $\sum_{t=k+1}^{j}sub(\tau_q[i], \tau_d[t])$ as $sub(i,k+1:j)$. For $\forall j\geq 2$ when $i=2$, we have
   {\small \begin{eqnarray}
        C_{2,j}&=&\mathop{\min}\limits_{1\leq k < j}\mathop{\min}\limits_{k\leq t < j}C_{1,k}+sub(1,k+1:t)+sub(2,t+1:j)\notag \\
        &=&\mathop{\min}\limits_{1\leq t < j}\mathop{\min}\limits_{1\leq k \leq t}{sub(1,k:t)+sub(2,t+1:j)}\notag \\
        &=&\mathop{\min}\limits_{1\leq t < j}{sub(\tau_q[1],\tau_d[t])+sub(2,t+1:j)}\notag \\
        &=&\mathop{\min}\limits_{1\leq t < j}{C_{1,t}+\sum_{k=t+1}^{j}{sub(\tau_q[2],\tau_d[k])}}\notag\\
        &=&\mathop{\min}\limits_{1\leq k < j}{C_{1,k}+\sum_{t=k+1}^{j}{sub(\tau_q[2],\tau_d[t])}}\notag
    \end{eqnarray}}
    Suppose that when $i=h-1$, we have $C_{h-1,j}=\mathop{\min}\limits_{1\leq k < j}C_{h-2,k}+\sum_{t=k+1}^{j}sub(\tau_q[h-1], \tau_d[t])=\mathop{\min}\limits_{1\leq k < j}C_{h-2,k}+sub(h-1,k+1:j)$. Next, we have to prove that the theorem also holds when $i=h$.
   {\small \begin{eqnarray}
        C_{h,j}&=&\mathop{\min}\limits_{1\leq k < j}\mathop{\min}\limits_{k\leq t < j}C_{h-1,k}+sub(h-1,k+1:t) + sub(h,t+1:j)\notag \\
        &=&\mathop{\min}\limits_{1\leq t < j}\mathop{\min}\limits_{1\leq k \leq t}C_{h-1,k}+sub(h-1,k+1:t) + sub(h,t+1:j)\notag \\
        &=&\mathop{\min}\limits_{1\leq t < j}\mathop{\min}\limits_{1\leq k \leq t}\mathop{\min}\limits_{1\leq l < k}C_{h-2,l}+sub(h-1,l+1:k) \notag\\
        &&+ sub(h-1,k+1:t) + sub(h,t+1:j)\notag \\
        &=& \mathop{\min}\limits_{1\leq t < j}\mathop{\min}\limits_{1\leq l < t}C_{h-2,l} + sub(h-1,l+1:t)+sub(h,t+1:j) \notag \\
        &=&\mathop{\min}\limits_{1\leq t < j}C_{h-1,t}+sub(h,t+1:j)\notag \\
        &=&\mathop{\min}\limits_{1\leq k < j}C_{h-1,k}+\sum_{t=k+1}^{j}sub(\tau_q[h], \tau_d[t])\notag 
    \end{eqnarray}}
    The above analysis shows that the theorem holds when $i=2$ and the theorem holds when $i=h-1$ can infer that the theorem holds when $i=h$. Therefore, the theorem holds.
\end{proof}
After obtaining the expression for $C_{i,j}$ from the theorem \ref{the:simplify}, we can further simplify it.
{\small\begin{eqnarray}
    C_{i,j}&=&\mathop{\min}\limits_{1\leq k < j}C_{i-1,k}+\sum_{t=k+1}^{j}sub(\tau_q[i], \tau_d[t])\notag\\
    &=&\min\{\mathop{\min}\limits_{1\leq k < j-1}C_{i-1,k}+\sum_{t=k+1}^{j-1}sub(\tau_q[i], \tau_d[t]), \notag\\
    &&C_{i-1,j-1}\}+sub(\tau_q[i], \tau_d[j])\notag \\
    &=&\min\{C_{i,j-1},C_{i-1,j-1}\}+sub(\tau_q[i], \tau_d[j])\notag
\end{eqnarray}}
Finally, integrating all the previous analysis results, we can get the computational expression of $C_{i,j}$. With the equation \ref{eq:dtw}, we can quickly adapt the algorithm \ref{algo:efficiencyA} to get the optimal subtrajectory query algorithm with DTW as the distance function.
{\small\begin{equation}
    C_{i,j}=\left\{
    \begin{array}{ll}
    sub(\tau_q[i],\tau_d[j]), & i=1 \\
    C_{i-1,j}+sub(\tau_q[i],\tau_d[1]), & j=1,i\neq1 \\
    \min\{C_{i-1,j},C_{i,j-1},C_{i-1,j-1}\}\\
    +sub\left(\tau_q[i],\tau_d[j]\right),& otherwise
    \end{array}
    \right.
    \label{eq:dtw}
\end{equation}}

\subsection{Other Similarity Functions}
\label{sec:other}
In addition to DTW and WED, our method is also valid for other order-insensitive distance functions. EDR and ERP are specific cases of WED functions; therefore, we only need to define $sub$, $ins$, and $del$ in Equation \ref{eq:wed_cal}.
We denote the euclidean distance between two points $\tau_q[i]$ and $\tau_d[j]$ as $d(\tau_q[i], \tau_d[j])$. We can convert WED to ERP and EDR by defining $sub$, $ins$ and $del$: (i) ERP. We can convert WED into ERP by making $sub(\tau_q[i], \tau_d[j])=d(\tau_q[i], \tau_d[j])$, $del(\tau_q[i])=d(\tau_q[i], q_c)$, $ins(\tau_d[j])=d(\tau_d[j], q_c)$ into ERP, where $q_c$ is a fixed point on the map (e.g., the center of the region). (ii) EDR. $ins(\tau_d[j])$ and $del(\tau_q[i])$ in EDR are both 1, while $sub(\tau_q[i], \tau_d[j])$ takes a value of 0 if and only if $d(\tau_d[j], q_c) < \epsilon$ holds; otherwise, $sub(\tau_q[i], \tau_d[j])=1$.

FD is similar to DTW. In the same way, we can obtain the expressions for $C_{i,j}$ when FD is the distance function.
\begin{equation}
    C_{i,j}=\left\{
    \begin{array}{ll}
    sub\left(\tau_q[i],\tau_d[j]\right), & i=1 \\
    \max\left\{C_{i-1,j},sub(\tau_q[i],\tau_d[1])\right\}, & j=1,i\neq1 \\
    \max\{\min\{C_{i-1,j},C_{i,j-1},C_{i-1,j-1}\},\\
    sub\left(\tau_q[i],\tau_d[j]\right)\},& otherwise
    \end{array}
    \right.
    \label{eq:dtw}
\end{equation}
When the order-insensitive distance functions are used as the trajectory distance functions, the calculation of the conversation cost does not depend on the position of the current point in the trajectory.


Our method does not apply to the subtrajectory search problem when order-sensitive distance function (e.g., LCSS) is used as the distance function between trajectories. The reason is that we do not consider the position from which the subtrajectory starts when computing $C_{i,j}$. When $\tau_q[i]$ matches $\tau_d[j]$, the cost of converting $\tau_q[i]$ to $\tau_d[j]$ should be only related to the matching relationship between $\tau_q[i-1]$ and $\tau_d[k]$ ($1\leq k \leq j$). However, when LCSS is used as the distance function, the cost of converting $\tau_q[i]$ to $\tau_d[j]$ is also related to the matching relation of $\tau_q[1]$, i.e., the starting position of the subtrajectory. The starting position of the subtrajectories has a great influence on judging the distance between the points in two trajectories when LCSS is used as the distance function. Therefore, our algorithm is not suitable for a class of distance functions that considers the position of points in the trajectory, such as LCSS.

==> pruneAlgorithm.tex <==
\section{Prune Principle}
\label{sec:prune}


eryIn the previous section, we proposed an algorithm with the time complexity of $O(mn)$ to find the subtrajectory with the minimum distance for the query trajectory in a data trajectory. The computation complexity for solving the SSS problem is thus optimized to $O(Nmn)$. Although the Algorithm \ref{algo:efficiencyA} is efficient enough to complete a search within $10ms$, considering a large number of data trajectories in the database (i.e., usually millions of data), the time to find the optimal subtrajectory from the database is about 15 minutes to half an hour for a given query trajectory. This is still not affordable for most of the applications. In practice, most of the data trajectories in the database are far distant from the query trajectory. We assume that only $Q$ data trajectories are ``similar'' for each query trajectory when the number of data trajectories is $N$, then it is meaningless to search for the optimal subtrajectories from other data trajectories. 
% 在本节中，我们设计了两个模块来过滤到

\noindent\textbf{Filter with Key Points (FKP)}
For each point $\tau_q[i]$ in the query trajectory $\tau_q$, we can convert it to a point in the data trajectory by substitution or deletion. Without considering other points, each point has a minimum cost of conversion. We use $minCost(\tau_q[i],\tau_d)$ to denote the lower bound of the cost of converting $\tau_q[i]$ to a point in $\tau_d$ and we define $minCost(\tau_q[i],\tau_d)$ as follows.
{\small\begin{eqnarray}
    minCost(\tau_q[i],\tau_d)=\min\{del(\tau_q[i]), \mathop{\min}\limits_{1\leq j\leq \tau_d.l}sub(\tau_q[i],\tau_d[j])\} \notag
\end{eqnarray}}
% Next, we introduce the lower bound on the conversion cost by the Theorem \ref{the:lbocc}.
% \begin{theorem}[Lower Bound of Cost]
%     \label{the:lbocc}
%     We denote {\small$minCost(\tau_q,\tau_d)$} as {\small$\sum_{i=1}^{\tau_q.l}minCost(\tau_q[i],\tau_d )$} and {\small$minCost(\tau_q,\tau_d)$} is the lower bound on the cost of converting $\tau_q$ to $\tau_d$, i.e., {\scriptsize$minCost(\tau_q,\tau_d)\leq \mathop{\min}\limits_{1\leq j\leq \tau_d.l}C_{\tau_q.l,j}$}.
% \end{theorem}
% \begin{proof}
%     We use WED as an example to prove this theorem using mathematical induction.
    
%     (i) When $i=1$, we have {\scriptsize$minCost(\tau_q[1:i],\tau_d)\leq \mathop{\min}\limits_{1\leq j\leq \tau_d.l}sub(\tau_q[1],\tau_d[j])=\mathop{\min}\limits_{1\leq j\leq \tau_d.l}C_{\tau_q.l,j}$}.
    
%     (ii) Suppose when $i=k-1$, we have {\small$minCost(\tau_q[1:k-1],\tau_d)\leq \mathop{\min}\limits_{1\leq j\leq \tau_d.l}C_{k-1,j}$}. We will discuss the case when $i=k$ in two scenarios. If $j=1$, then {\small$minCost(\tau_q[1:k],\tau_d)=minCost(\tau_q[1:k-1],\tau_d)+minCost(\tau_q[k],\tau_d)$}. Considering that {\small$minCost(\tau_q[1:k-1],\tau_d)<C_{k-1,1}$} and {\small$minCost(\tau_q[1:k-1],\tau_d)<del(\tau_q[1:i-1])$}, we have {\small$minCost(\tau_q[1:k],\tau_d)\leq \min\{C_{i-1,j}+del(\tau_q[i]), sub(\tau_q[i],\tau_d[1])+del(\tau_q[1:i-1])\}=C_{k,1}$}. For each {\small$\forall j\neq 1$}, we have 
%    {\small \begin{eqnarray}
%         &&minCost(\tau_q[1:k],\tau_d) \notag \\
%         &=&minCost(\tau_q[1:k-1],\tau_d) +minCost(\tau_q[k],\tau_d)\notag \\
%         &\leq& \mathop{\min}\limits_{1\leq t\leq j}C_{k-1,t}+sub(\tau_q[i],\tau_d[j]) \notag \\
%         &\leq&C_{k,j} \notag
%     \end{eqnarray}}
%     Thus, we can obtain $minCost(\tau_q[1:k],\tau_d)\leq \mathop{\min}\limits_{1\leq j\leq \tau_d.l}C_{k,j}$.

%     Finally, by combining (i) and (ii), the theorem \ref{the:lbocc} is proved.
% \end{proof}

% \begin{figure}
% 	\begin{small}
% 		\begin{center}
% 			\includegraphics[width=0.30\textwidth]{../figures/pruningExample.png}
% 		\end{center}
% 		\caption{Pruning Example}
% 		\label{fig:pruningExample}
% 	\end{small}
% \end{figure}

Nevertheless, we cannot directly compute $minCost(\tau_q,\tau_d)$ in practical applications. It is because the time complexity of computing $minCost(\tau_q,\tau_d)$ is $O(\tau_q.l\cdot\tau_d.l)$, which is the same as the time complexity of computing the optimal subtrajectory directly. Fortunately, we can approximate $minCost(\tau_q,\tau_d)$ due to the continuity of trajectory. In reality, the position of an object cannot change dramatically in a short time, thus the location of a point in a trajectory is close to the location of its neighboring points. Based on the continuity of the trajectory, we can select key points $Key(\tau_q)(=\{\tau_q[e_1],\tau_q[e_2],\dots,\tau_q[e_K]\})$ from the original query trajectory. Based on these key points, we can compute the estimation of $minCost(\tau_q,\tau_d)$ and denote it by $minCost_e(\tau_q,\tau_d)$ as follows.
{\small\begin{equation}
minCost_e(\tau_q,\tau_d)=r\sum_{\tau_q[e_i]\in Key(\tau_q)}minCost(\tau_q[e_i],\tau_d) \label{eq:e2}
\end{equation}}
Here, $r=\frac{|Key(\tau_d)|}{\tau_d.l}$ denoting the ratio of key points selected from the query trajectory. The selection of key points $Key(\tau_q)$ affects the accuracy of estimation and we uniformly select points from $\tau_q$ in this paper. The more key points in $Key(\tau_q)$, the more accurate the estimation of $minCost(\tau_q,\tau_d)$ will be. However, the time complexity of the computation also increases as $Key(\tau_q)$ increases. Therefore, we need to choose as few key points as possible while ensuring the estimation accuracy as much as possible.



\begin{algorithm}[t]
	{\small
	\DontPrintSemicolon
	\KwIn{\small a query trajectory $\tau_q$, data trajectories $\{\tau_d^{(1)},\tau_d^{(2)},\dots,\tau_d^{(N)}\}$}
	\KwOut{\small the optimal subtrajectory $\tau_d^{(k^{*})}[i^{*}:j^{*}]$ for the query trajectory $\tau_q$}
    $\tau_d^{(*)}[i^{*}:j^{*}]\gets \{\}$\;
    \ForAll{$1\leq k \leq N$}{
        For each point in the data trajectory $\tau_d^{(k)}$, we compute $H(\tau_d^{(k)}[j])$ according to the Equation \ref{equ:eq4}\;\label{line:3}
        
        According to the equation \ref{equ:eq3}, we can compute $close(\tau_q,\tau_d^{(k)})$ for each query trajectory $\tau_q$\;
        
        \ForAll{$1\leq t \leq M$}{
            \eIf{$result = (-1,-1,-1)$ }{
                $\tau_d^{(k)}[i^{k}:j^{k}]\gets CMA(\tau_q,\tau_d^{(k)})$\;
                $\tau_d^{(*)}[i^{*}:j^{*}]\gets \tau_d^{(k)}[i^{k}:j^{k}]$\;
            }{
                \If{$close(\tau_q,\tau_d^{(k)})>\mu \cdot \tau_q.l$}{
                    calculate the estimation of the lower bound $minCost_e(\tau_q,\tau_d^{(k)})$ by Equation \ref{eq:e2}\;
                    \If{$minCost_e(\tau_q,\tau_d^{(k)})<\Theta(\tau_q,\tau_d^{(*)}[i^{*}:j^{*}])$}{
                        \label{line:14}
                        $\tau_d^{(k)}[i^{k}:j^{k}]\gets CMA(\tau_q,\tau_d^{(k)})$\;
                        \If{$\Theta(\tau_q,\tau_d^{(k)}[i^{k}:j^{k}])<\Theta(\tau_q,\tau_d^{(*)}[i^{*}:j^{*}])$}{
                            $\tau_d^{(*)}[i^{*}:j^{*}]\gets \tau_d^{(k)}[i^{k}:j^{k}]$\;
                        }
                    }
                }
            }
        }
    }
    \Return{$\tau_d^{(*)}[i^{*}:j^{*}]$}
	\caption{\small Pruning Algorithm}
	\label{algo:efficiencyC}}
\end{algorithm}


\noindent\textbf{Grid Based Pruning (GBP)}
% Even though we can estimate the lower bound of the distance between the query trajectory and the subtrajectories of the data trajectory by selecting some key points, the time complexity of pruning increases as the number of query trajectories $M$ and $|Key(\tau_q)|$ increases. Therefore, we will introduce a grid-based pruning strategy in this section. 
The basic idea is to divide the whole map into multiple grids, and we use a hash table to record the grid where the key points of each trajectory are located. Then, for each point in the data trajectory, we only check all the key points of the query trajectory located within its grid and neighbor grids using the hash table. Finally, if a query trajectory has multiple key points around a given data trajectory, it is similar to the current data trajectory, and it is necessary to search the current data trajectory. Let us explain the details of the algorithm in the following part.



We divide the map into a square grid with $\varepsilon $ as side lengths. For a point $\tau_d^{(k)}[j]$ in the data trajectory, we denote the grid it locates in as $g(\tau_d^{(k)}[j])$. Each grid is surrounded by 8 neighboring grids and we denote the set consisting of the grid $g(\tau_d^{(k)}[j])$ and its neighboring grids as $B(\tau_d^{(k)}[j])$. We consider $\tau_d^{(k)}[j]$ to be \textit{close} to the points in the grid it is located in and its neighboring grids, i.e., a point $\tau_q^{(t)}[i]$ is close to $\tau_d^{(k)}[j]$ if and only if $g(\tau_q^{(t)}[i]) \in B(\tau_d^{(k)}[j])$. If there exists a point in a query trajectory that is close to $\tau_d^{(k)}[j]$, then we consider this query trajectory to be close to $\tau_d^{(k)}[j]$. Meanwhile, we denote the set formed by the points of all query trajectories close to $\tau_d^{(k)}[j]$ as $H(\tau_d^{(k)}[j])$.

{\small\begin{eqnarray}
    H(\tau_d^{(k)}[j])=\{\tau_q^{(t)}[i]|g(\tau_q^{(t)}[i]) \in B(\tau_d^{(k)}[j])\} \label{equ:eq4}
\end{eqnarray}}

Given a data trajectory $\tau_d^{(k)}$, we can count how many points in the query trajectory $\tau_q$ are close to that query trajectory and denote it as $close(\tau_q,\tau_d^{(k)})$, that is, 
{\small\begin{eqnarray}
close(\tau_q,\tau_d^{(k)})=\left|\left\{\tau_q[i]\left|\tau_q[i] \in \mathop{\cup}\limits_{1\leq j \leq \tau_d^{(k)}.l}H(\tau_d^{(k)}[j])\right.\right\}\right| \label{equ:eq3}
\end{eqnarray}}
The larger $close(\tau_q,\tau_d^{(k)})$ means that more points of the query trajectory are distributed around the data trajectory $\tau_d^{(k)}$, then there is likely a segment of sub-trajectories in $\tau_d^{(k)}$ that are similar to $\tau_q$. We define a constant $\mu$ ($0<\mu<1$) and we call the algorithm \ref{algo:efficiencyA} to search for the optimal sub-trajectory in $\tau_d^{(k)}$ whenever $close(\tau_q,\tau_d^{(k)})\geq \mu \cdot \tau_q.l$.

% \begin{figure}
% 	\begin{small}
% 		\begin{center}
% 			\includegraphics[width=0.30\textwidth]{../figures/complexity.png}
% 		\end{center}
% 		\caption{Complexity Analysis}
% 		\label{fig:complexityanalysis}
% 	\end{small}
% \end{figure}

% \begin{example}
%     $H(\tau_d^{(k)}[j])$ denotes the set consisting of all points in the neighbor of $\tau_d^{(k)}[j]$. Figure k shows one data trajectory and three query trajectories. The point $\tau_d^{(1)}[4]$ is surrounded by points $\tau_q^{(2)}[1],\tau_q^{(1)}[3]$ and $\tau_q^{(3)}[1]$; thus, $H(\tau_d^{(1)}[4])=\{\tau_q^{(2)}[1],\tau_q^{(1)}[3],$ $\tau_q^{(3)}[1]\}$.  Besides, we have $H(\tau_d^{(1)}[5])=\{\tau_q^{(2)}[2],\tau_q^{(2)}[3],\tau_q^{(3)}[1],$ $\tau_q^{(3)}[2]\}$. $close(\tau_q^{(t)},\tau_d^{(k)})$ denotes the set of all points in $\tau_q^{(t)}$ appearing in the neighbor of $\tau_d^{(k)}$. For the query trajectory $\tau_q^{(1)}$, all its points are near at least one point of the data trajectory $\tau_d^{(1)}$. Thus, $close(\tau_q^{(1)},\tau_d^{(1)})=\{\tau_q^{(1)}[1],\tau_q^{(1)}[2],\tau_q^{(1)}[3]\}$. Similarly, we have $close(\tau_q^{(1)},\tau_d^{(3)})=\{\tau_q^{(3)}[1],\tau_q^{(3)}[2],\tau_q^{(3)}[3]\}$. Thus, when we set $\mu$ to 1, only $\tau_q^{(1)}$ and $\tau_q^{(2)}$ are considered similar to $\tau_d^{(1)}$. We will call the algorithm \ref{algo:efficiencyA} to search the subtrajectories from $\tau_d^{(1)}$ with the closest distance to $\tau_q^{(1)}$ and $\tau_q^{(2)}$.
% \end{example}

\noindent\textbf{Complexity.} By using the hash table, we can find the points in its neighboring grid for each $\tau_d^{(k)}[j]$ in a constant time. Thus the time complexity of computing $H(\tau_d^{(k)}[j])$ is $O(1)$, making the time complexity of computing for each point in the data trajectory $O(\tau_d^{(k)}.l)$. On the other hand, the computational complexity of Equation \ref{equ:eq3} depends mainly on the number of points in the query trajectory around the data trajectory, which is much smaller than $\tau_d^{(k)}.l$. Therefore, the pruning complexity is $O(Nn)$ in total if the average length of the data trajectories is $n$. Suppose the average length of the query trajectory is $m$. Since we select key points from the query trajectory at a certain ratio $r$, the number of key points is $mr$. Thus, the time complexity of computing the distance lower bound is $mrQn$, where $Q$ denote the count of trajectories satisfying $close(\tau_q,\tau_d^{(k)})>\mu \cdot \tau_q.l$. Finally, the time complexity of the algorithm \ref{algo:efficiencyC} is $O(Nn+mrQn+Q'mn)$, where $Q'$ denotes the count of trajectories satisfying line \ref{line:14}, and we have $N\gg Q\gg Q'$.

